Integrable RCS as a proposed replacement for Fermilab Booster

Integrable optics is an innovation in particle accelerator design that potentially enables a greater betatron tune spread and damps collective instabilities. An integrable rapid-cycling synchrotron (RCS) would be an effective replacement for the Fermilab Booster, as part of a plan to reach multi-MW beam power at 120 GeV for the Fermilab high-energy neutrino program. We provide an example integrable lattice with features of a modern RCS - dispersion-free drifts, low momentum compaction factor, superperiodicity, chromaticity correction, bounded beta functions, and separate-function magnets.

==> bib.tex <==
@ARTICLE{Danilov,
   AUTHOR  = {V. Danilov and S. Nagaitsev},
   TITLE   = {Nonlinear accelerator lattices with one and two analytic invariants},  
   YEAR    = {2010},
   JOURNAL = "Phys. Rev. ST Accel. Beams",
   VOLUME  = {13},
   PAGES   = {084002}
}

@INPROCEEDINGS{Valishev,
	author    = "A. Valishev and S. Nagaitsev and D. Shatilov and V. Danilov",
	title     = "BEAM PHYSICS OF {I}NTEGRABLE {O}PTICS {T}EST {A}CCELERATOR AT {F}ERMILAB ",
	booktitle = "Proceedings of IPAC2012",
	year      = "2012"
}

@INPROCEEDINGS{Ruisard,
	author    = "K. Ruisard and H. Baumgartner and B. Beaudoin and I. Haber and D. Matthews and T. Koeth",
	title     = "EARLY TESTS AND SIMULATION OF QUASI-INTEGRABLE OCTUPOLE LATTICES AT THE {U}NIVERSITY OF {M}ARYLAND {E}LECTRON {R}ING",
	booktitle = "Proceedings of HB2016",
	year      = "2016"
}

@INPROCEEDINGS{Prebys,
	author    = "E.J. Prebys and others",
	title     = "LONG TERM PLANS TO INCREASE {F}ERMILAB’S PROTON INTENSITY TO MEET THE NEEDS OF THE LONG BASELINE NEUTRINO PROGRAM",
	booktitle = "Proceedings of IPAC2016",
	year      = "2016"
}

@TECHREPORT{PIP2,
     author       = "Paul Derwent and others",
     title        = "{P}roton {I}mprovement {P}lan-{II}",
     institution  = "Fermi National Accelerator Facility",
     year         = "2013",
     PAGES        = "Project X-doc-1232"
}

@misc{DUNE,
  title        = "{L}ong-{B}aseline {N}eutrino {F}acility ({LBNF}) and {D}eep {U}nderground {N}eutrino {E}xperiment ({DUNE}) {C}onceptual {D}esign {R}eport",
  year         = "2015",
}

@misc{P5,
  title        = "{R}eport of the {P}article {P}hysics {P}roject {P}rioritization {P}anel",
  year         = "2014",
}

@INPROCEEDINGS{Lebedev,
	author    = "V.A. Lebedev and J.-F. Ostiguy and C.M. Bhat",
	title     = "BEAM ACCELERATION AND TRANSITION CROSSING IN THE {F}ERMILAB {B}OOSTER",
	booktitle = "Proceedings of HB2016",
	year      = "2016"
}

@INPROCEEDINGS{Antipov,
	author    = "S.A. Antipov and P. Adamson and S. Nagaitsev and M.-J. Yang",
	title     = "STUDY OF FAST INSTABILITY IN {F}ERMILAB {R}ECYCLER",
	booktitle = "Proceedings of IPAC2016",
	year      = "2016"
}

@INPROCEEDINGS{Pellico,
	author    = "W. Pellico and K. Domann and F.G. Garcia and K. Gollwitzer and K. Seiya and B. Zwaska",
	title     = "{FNAL} - {T}he {P}roton {I}mprovement {P}lan ({PIP})",
	booktitle = "Proceedings of IPAC2014",
	year      = "2014"
}

@TECHREPORT{Bruhwiler,
     author       = "D.L. Bruhwiler and others",
     title        = "Challenges to demonstrating integrable proton dynamics in {IOTA}",
     institution  = "Fermi National Accelerator Laboratory",
     year         = "2016",
     PAGES        = "Beams-doc-5167-v1"
}

@ARTICLE{Brown,
   AUTHOR  = {B.C. Brown and others},
   TITLE   = {{F}ermilab main injector: {H}igh intensity operation and beam loss control},  
   YEAR    = {2013},
   JOURNAL = "Phys. Rev. ST Accel. Beams",
   VOLUME  = {16},
   PAGES   = {071001}
}

@ARTICLE{Eldred,
   AUTHOR  = {J. Eldred and R. Zwaska},
   TITLE   = {Enhanced Dynamical Stability with Harmonic Slip-stacking},  
   YEAR    = {2016},
   JOURNAL = "Phys. Rev. Accel. Beams",
   VOLUME  = {19},
   PAGES   = {104001}
}

@INPROCEEDINGS{Dixon,
	author    = "S. Dixon",
	title     = "Siting/Conventional Facilities Status",
	booktitle = "Presented at {M}arch 2016 {F}ermilab {PIP-
II} {M}achine {A}dvisory {C}ommittee {M}eeting",
	year      = "2016"
}

@ARTICLE{Tang,
   AUTHOR  = {J. Tang},
   TITLE   = {Rapid Cycling Synchrotrons and Accumulator Rings for High-Intensity Hadron Beams},  
   YEAR    = {2013},
   JOURNAL = "Rev. Accel. Sci. Technol.",
   VOLUME  = {06},
   PAGES   = {143}
}

@INPROCEEDINGS{Romanov,
	author    = "G. Romanov and others",
	title     = "PERPENDICULAR BIASED FERRITE TUNED CAVITIES FOR THE {F}ERMILAB {B}OOSTER",
	booktitle = "Proceedings of IPAC2014",
	year      = "2014"
}

@INPROCEEDINGS{Webb,
	author    = "S.D. Webb and D. Bruhwiler and A. Valishev and R. Kishek and S. Danilov and S. Nagaitsev",
	title     = "Chromaticity Considerations for Nonlinear Integrable Lattices",
	booktitle = "Proceedings of AAC2014, in press",
}

@INPROCEEDINGS{Cook,
	author    = "N. Cook and others",
	title     = "Understanding perturbations to nonlinear 
integrable optics in {IOTA}",
	booktitle = "paper in these Proceedings",
	year      = "2016"
}

@ARTICLE{JPARC,
   AUTHOR  = {H. Hotchi and others},
   TITLE   = {Beam loss reduction by injection painting in the 3-{G}eV rapid cycling synchrotron of the {J}apan {P}roton {A}ccelerator {R}esearch {C}omplex},  
   YEAR    = {2012},
   JOURNAL = "Phys. Rev. ST Accel. Beams",
   VOLUME  = {15},
   PAGES   = {040402}
}

@ARTICLE{Pham,
   AUTHOR  = {A. Pham and S.Y. Lee and K.Y. Ng},
   TITLE   = {Method of phase space beam dilution utilizing bounded chaos generated by rf phase modulation},  
   YEAR    = {2015},
   JOURNAL = "Phys. Rev. ST Accel. Beams",
   VOLUME  = {18},
   PAGES   = {124001}
}

